BOSS: A Blockchain Off-State Sharing System

Blockchain has been applied to data sharing to ensure the integrity of data and chain of custody. Sharing big data such as large biomedical data files is a challenge to blockchain systems since the ledger is not designed to maintain big files, access control is an issue, and users may be dishonest. We call big data such as big files stored outside of a ledger that includes the blockchain and world state at a blockchain node as "off-state" and propose an off-state sharing protocol for a blockchain system to share big data between pairs of nodes. In our protocol, only encrypted files are transferred. The cryptographic key is stored in the world state in a secure way and can be accessed only by authorized parties. A receiver has to request the corresponding cryptographic key from the sender to decrypt such encrypted files. All requests are run through transactions to establish reliable chain of custody. We design and implement a prototypical blockchain off-state sharing system, BOSS, with Hyperledger Fabric. Extensive experiments were performed to validate the feasibility and performance of BOSS.

==> CNS2021_File_sharing_arXiv/sections/sec1_introduction.tex <==
\section{Introduction}

A blockchain system can build trust in the data that it maintains without a centralized authority. Data in conventional blockchain systems is often stored in a ledger, which includes a world state and a blockchain. The world state stores the current system state such as the user cryptocurrency balance in Bitcoin \cite{antonopoulos2014mastering} and the blockchain saves all transaction history, which contains operations on the world state and/or the data used to update the world state. The whole transaction history produces the current state values and can work as auditing evidence. The ledger is often synchronized across all nodes.

Blockchain has been applied to a variety of data sharing applications such as healthcare.
A blockchain data sharing system can prevent information tampering for the purpose of auditing and establish the chain of custody, which refers to the documentation that records the sequence of custody, transfer, and other operations on the data.
In these systems, shared data is stored in the world state database. Users set or get shared data through proposing transactions to the blockchain system.

The existing blockchain frameworks cannot be directly applied to big file sharing.
Big files can be scientific and biomedical data being collected and processed. Sharing such data allows independent verification of published scientific results and enhances opportunities for new discoveries. With concerns of intellectual property (IP) theft and industrial espionage, we desire secure and trustworthy big file sharing systems that record the chain of custody of the big files. However, given the storage design of the ledger, it is impractical to store big files in the world state and to use transactions to carry big files. A blockchain system often maintains the same ledger across all nodes. However, because of privacy, IP and storage concerns, owners may not want to share those big files across all nodes. 

A token based data sharing blockchain system has been briefly discussed in related work \cite{zhang2018fhirchain}. Shared data is stored outside the blockchain system at a data center.
This system has the following issues: (i) It requires a centralized and trusted data center. (ii) No actual protocols using tokens are documented. (iii) The data center based approach is not flexible. In scenarios such as file sharing in biomedical fields, researchers may want to share data between each other's computers directly. There is no detail of the token based sharing protocol in \cite{zhang2018fhirchain}.

In this paper, we propose a novel big file sharing model. Our major contributions can be summarized as follows.

\begin{enumerate}
\item We introduce a new concept ``off-state" to a blockchain system. A blockchain node may maintain a separate storage from the ledger to store off-states such as big files, which are outside of the ledger, particularly the world state. Off-states do not need to be synchronized across all nodes. Smart contracts manage sharing of off-states such as big files.

\item To ensure the integrity and chain of custody of off-states, we propose a novel off-state sharing protocol. Off-sates are encrypted and signed before sharing. The cryptographic key is stored in the world state database and users have to request the key through transactions in order to decrypt the transferred files. Mechanisms such as private data collection (PDC) in Hyperledger Fabric \cite{androulaki2018hyperledger} can be used to ensure that the cryptographic key is kept private and not publicly disclosed. These mechanisms also defeat dishonest users.

\item We implement a prototypical blockchain off-state sharing system (BOSS) with Hyperleger Fabric running our off-state data sharing protocol. Extensive experiments are performed to evaluate BOSS' feasibility and performance such as latency of the big file transfer between pairs of blockchain nodes and parallel file transfer.
%We measure the latency of involved transactions and the latency of one file sharing event, and analyze how the file size and the parallel number affect the latency. 
%Base on the results, we further propose a load balance scheme to optimize the latency in parallel cases.

\end{enumerate}


The rest of this paper is organized as follows. Section \ref{sec::background} introduces the background knowledge. Section \ref{sec::system Model} introduces the off-state sharing system model. The off-state sharing protocol is presented in Section \ref{sec::Integration_Scheme}. We evaluate the prototypical off-state sharing system, BOSS, in Section \ref{sec::Evaluations}. We discuss a few related topics such as the execution timeout of chaincode (i.e. smart contract in Hyperledger Fabric) in Section \ref{sec::discussion}. Section \ref{sec::related_work} presents the related work. We conclude this paper in Section \ref{sec::Conclusion}.



==> CNS2021_File_sharing_arXiv/sections/sec2_background.tex <==
\section{Background}
\label{sec::background}

In this section, we introduce the data in blockchain systems, storage limitations of a ledger, and Hyperledger Fabric, which is a permissioned blockchain framework. For brevity, we will call Hyperledger Fabric as Fabric in the rest of the paper.

\subsection{Data in Conventional Blockchain Systems}
\label{sec::world_state}

A blockchain system is essentially a state machine replicated across different nodes \cite{buterin2014next}. The state machine can be formally defined in Formula (\ref{eqn::enctypt_aes}).
\begin{eqnarray}
APPLY(S, Tx) \rightarrow S' or ERROR,
\label{eqn::enctypt_aes}
\end{eqnarray}
where the state transition function $APPLY(.)$ takes a state $S$ and a transaction $Tx$ and outputs a new state $S'$ or an error. 
%\shan{The state is stored in a ledger.}
A ledger includes a world state and a blockchain. 
The world state stores the current state. The blockchain stores all historical transactions.
In Bitcoin \cite{antonopoulos2014mastering}, the world state is the user cryptocurrency balance recorded in the UTXO (unspent transaction output) field of transactions.
State transitions are cryptocurrency transfers. 
%Fig. \ref{fig::state_machine} shows a state machine example of Bitcoin.
In Ethereum \cite{buterin2014next}, the world state is made up of ``accounts". An account contains the cryptocurrency balance, code and data in smart contracts and others. State transitions are direct transfers of values and information between accounts controlled by smart contracts. In Fabric \cite{androulaki2018hyperledger}, each peer node maintains a world state database. A transaction records the operation of invoking a function in smart contract, called chaincode in Fabric, which may work on the world state. \looseness=-1

\subsection{Storage Limitations of Conventional Blockchain Systems}
\label{sec::Storage_Limitations}

In current blockchain frameworks, the data size and type in ledgers are limited. 
%Both the world state and the blockchain have storage limitations.
We now show the limitations in three popular blockchain frameworks, Bitcoin, Ethereum and Fabric. 
% \looseness=-1

\subsubsection{\textbf{World State Storage Limitation}}
% The size and type of the data in world state is limited. 

In Bitcoin, the world state UTXOs are just values in transactions indicating the Bitcoin balance. It's impossible to store large files in UTXOs.

In Ethereum, the world state consists of user accounts and contract accounts. A user account only records the Ether balance of the user. The contract account can store pairs of keys and values of 32 bytes used by the smart contract \cite{EthereumBuildersGuideline}.
Ethereum is not designed to store big files.

In Fabric, the world state is stored in a database, i.e. LevelDB or CouchDB. LevelDB can only store simple key-value pairs. CouchDB can store data in the JSON format, but limits the maximum document body size to 8M bytes \cite{couchDB_Doc}. Fabric cannot store big files either.

\subsubsection{\textbf{Transaction and Block Size Limitation}}

In Bitcoin, to prevent attacks like DoS attacks and memory exhaustion attacks, it restricts the block size to 1MB and transactions greater than 100 KB are considered non-standard \cite{BitcoinWeakness,BitcoinForum}.

In Ethereum, the {\em gas} consumed by a transaction is related to the size of the data stored in the world state. It is quite expensive to store big data. According to the yellow paper \cite{EthYellowPaper}, it requires 16 gas units for storing every non-zero byte of data for a transaction. Storing 1MB ($1024 \times 1024 = 1048576 \ bytes$) data requires 16,777,216 gas units in addition to other fees. Each block has a block gas limit, which limits the block size too.
The current block gas limit is 12,491,593 gas units/block \cite{GasLimit}.
It means a block can maximally store about 0.74MB data ($12491593 \div 16777216 \approx 0.74$).\looseness=-1

In Fabric, the preferred maximum size of each transaction is 512KB while the absolute maximum transaction size is 99MB. Nodes in Fabric adopt the {\em grpc} communication protocol. The maximum inbound grpc message size is 100MB \cite{HyperledgerJavazAPI}. Large transactions will decrease the system performance in terms of transaction throughput \cite{gorenflo2020fastfabric}. 
\looseness=-1

\subsection{Hyperledger Fabric}
\label{sec::hyperledger_fabric}

Fabric \cite{androulaki2018hyperledger} is a popular permissioned blockchain framework.
%A consortium of organizations build the system together. Only authorized participants can involve in a Hyperledger Fabric system. 
It decouples the tasks of a node in blockchain systems such as Ethereum \cite{buterin2014next} into three types of nodes, i.e. peers, orderers and clients in charge of different tasks. Peers maintain ledgers and smart contracts.
%\shan{Different nodes are responsible for different tasks in a transaction lifecycle.}
%\sout{A transaction is proposed by a client, then endorsed by peers, packaged into a block by orderers, and finally verified and stored into the ledger by peers. A valid transaction need to collect enough endorsements from peers, i.e. endorsers, specified by an endorsement policy.} 

%\shan{I move the transaction workflow from the subsection end here.}
\textit{Transaction Workflow:}
\label{subsubsec::FabricTransactionWorkflow}
Fabric adopts a three-phase ``execute-order-validate'' transaction workflow as shown in Fig. \ref{fig:txworkflow}: (1) A client/user proposes a transaction {\em proposal} to the endorsers, which are specific peers and specified by the endorsement policy; (2) The endorsers execute the chaincode, sign the execution results, and return the results with corresponding signatures to the client as proposal responses; (3) If the returned execution results from different endorsers are the same, the client constructs a transaction, which contains both the transaction proposal, proposal response and a list of signatures (endorsements). The client
sends the transaction to the orderer nodes. (4) The orderer nodes collect multiple transactions within a time period, bundle them into a new block, and distribute the new block to all peers including both endorsers and non-endorsers. (5) All peers validate the transactions in the received new block. If all transactions are valid, each peer will update the world state according to execution results. After validating all transactions, each peer appends the new block to its local blockchain. 


\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{figures/fig_transaction_workflow.pdf}
\caption{Three-phase transaction workflow in Fabric
}
\label{fig:txworkflow} 
\end{figure}


Three features of Hyperledger Fabric enable it suitable to implement our blockchain big file sharing system.

\subsubsection{Fine-grained data isolation}
% \shan{As a permissioned blockchain system, there are multiple build-in access control mechanisms in Fabric to manage participants and data according to identities and pre-defined policies.}
The Fabric introduces a fine-grained data isolation mechnism, i.e., private data collection (PDC). PDC data is sensitive and shared by only a subset of peer nodes. A PDC is stored in the world state. Only PDC member peers can store the original data, while PDC non-member peers can only store the data hashes.
%It is quite suitable for storing the encryption keys in our integration mechanism. At first, the encryption key can be accessed only by the sender and then is shared between the sender and the receiver.

\subsubsection{Customizable smart contracts}
Smart contracts, also called chaincode in Fabric, do not need to be identical at all peers as long as the execution results across different endorser peers are the same. 
%It is quite appropriate for manage inconsistent off-state data across different nodes. 
Therefore, different peers can perform different roles and tasks.
%, such as some nodes perform as file senders and some nodes perform as file receivers. And according to Fig. \ref{fig::Module2}, in one file transfer event, different roles need perform different tasks. %The customizable smart contracts feature is crucial.

\subsubsection{Multi-level endorsement policy}
There are multiple levels of endorsement policies in Fabric. An endorsement policy stipulates which peers need perform as endorsers to endorse a transaction. Endorsing involves executing smart contracts and signing the execution results.
Each smart contract has a default chaincode-level endorsement policy that manages all public data and PDC data in the world state. A collection-level endorsement policy can be customized to specifically manage the PDC data. 
%If a collection-level policy is set, it will overwrite the endorsement policy for PDC. 
%Besides, a key-level endorsement policy can be customized to manage a specific entry in world state. The key-level endorsement policy has the highest priority. 
% The multi-level endorsement policy is flexible for managing \texttt{File Profile}, \texttt{Event} and \texttt{Encryption Key} entry in the same smart contract. Different entries need be managed using different endorsement policies as analysed in Section \ref{sec::Endorsement_Policy_Set}.



==> CNS2021_File_sharing_arXiv/sections/sec3_model.tex <==
\section{Off-State Data Sharing System Model}
\label{sec::system Model}

In this section, we first investigate the existing blockchain-based big file sharing systems and their drawbacks. We then present the challenges in big file sharing through blockchain systems, and finally propose a new big file sharing model through blockchain.

\subsection{State-of-the-art Blockchain Based Big File Sharing Systems}
\label{sec::Existing_System_Models_Analysis}

Fig. \ref{fig:exist_system_model2} shows a blockchain-based data sharing model utilizing access tokens \cite{zhang2018fhirchain}. 
A user proposes a transaction to request a token for data access. The transaction proposal triggers particular functions in the smart contract, which returns an access token to the user. 
The user then uses the access token to request the shared data from a data center, which is outside of the blockchain system. This data sharing model may be used for big file sharing.
%\shan{The token-based model has no storage limitations and can be used to share big files.}

The token based file sharing blockchain model has the following issues: (i) It requires a centralized and trusted data provider. 
The data center is controlled by the data provider.
The Blockchain system has no control over the actual data access and cannot know the status of data sharing, e.g. whether the data is actually shared. 
%Data access is not part of Blockchain systems, which cannot record the file sharing status into the blockchain for proof.
The integrity of chain of custody cannot be ensured and audited,
(ii) There is no detailed presentation of the actual protocol in \cite{zhang2018fhirchain}.
(iii) The data center based approach is not flexible. In scenarios such as file sharing in biomedical fields, data owners may want to share data between their workstations. 
\begin{figure}
\centering
\includegraphics[width=0.85\columnwidth]{figures/fig_system model outside data.pdf}
\caption{Token based blockchain data sharing system
}
\label{fig:exist_system_model2} 
\end{figure}


\subsection{Design Challenges}

We identify three challenges for a blockchain-based big file sharing system.

\subsubsection{Challenge 1---Storage Space Limitation}

Big files refer to files of large size, such as videos and biomedical data files.
Due to the storage limitations of ledgers as discussed in Section \ref{sec::Storage_Limitations}, it is impractical to store big files in ledgers or pack big files in transactions. 

\subsubsection{Challenge 2---Privacy Requirement}
\label{sec::challenge2}

Big files may be sensitive. The owner may not want to share with everyone and access control will be preferred.
However, in a conventional blockchain system, all nodes maintain the same data. Therefore, the blockchain system cannot be directly used for big file sharing.

\subsubsection{Challenge 3---Security Requirement}
\label{sec::challenge3}
In big file sharing, the receiver of the big files may be dishonest and may dishonestly deny she/he received the files from the owner.
%A sender may dishonestly claim she/he has transferred files or transfer wrong files.


\subsection{Off-State Sharing System Model}
\label{sec::off-stateConcept}

We introduce the concept of ``off-state", which is stored at blockchain nodes, but outside of ledgers, particularly the world state. For example, the off-state can be big files.
Therefore, we generalize big file sharing as off-state sharing. 
Off-states can be inconsistent across blockchain nodes and shared between pairs of nodes. Smart contracts at blockchain nodes can interact with off-states and perform the sharing operation. 

Fig. \ref{fig:system_model} shows our novel blockchain system model that can address the three challenges above for off-state data sharing. Each node maintains a world state database and an off-state storage space when needed. Nodes maintain their off-state data individually. Users propose transactions to trigger the smart contracts to transfer the files. The smart contracts at the sender node transfers off-state data to the receiver node through a file transfer protocol, not through transactions. 

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{figures/fig_system model off-state.pdf}
\caption{Blockchain-based off-state sharing model
}
\label{fig:system_model} 
\end{figure}

To summarize, we address the three challenges as follows.
\begin{itemize}
\item 
To address Challenge 1---storage space limitation, we introduce the concept of `off-state" and save big files off the ledger. 

\item To address Challenge 2---privacy requirement, our protocol allows off-states to be shared between pairs of nodes, not across all blockchain nodes. This feature saves storage space at nodes that do not need off-state data.

\item To address Challenge 3---security requirement, our protocol establishes the chain of custody of the off-state data and records auditing evidence in the blockchain.
\end{itemize}
We will present the detailed off-state data sharing protocol in Section \ref{sec::Integration_Scheme}.





%To Our off-state sharing protocol records the off-sate data sharing status into the blockchain.
%\red{The protocol records the file sending occurrence, file receiving occurrence and transferred results in multiple transactions for proof. This can be implemented by tightly bond the operations on off-state with operations on world state. With a reliable blockchain framework, operations on world state are bound to recorded in transactions. More design details are illustrated in the next section.}


==> CNS2021_File_sharing_arXiv/sections/sec4_method.tex <==
\section{Off-State Sharing Protocol}
\label{sec::Integration_Scheme}

Our protocol has two stages. In Stage 1, an owner prepares the files to be shared with users and uploads the files to sender peer nodes. 
In Stage 2, to establish the chain of custody, a sender peer transfers an encrypted file to a receiver peer and stores the symmetric encryption/decryption key (called encryption key for brevity in the rest of the paper) in the world state. A user has to request the encryption key through a transaction to get the key, decrypt the encrypted file and get the original file. These transactions establish the chain of custody.
In this section, we first present the two stages and then perform the security analysis. We use Fabric to present particular protocol details and discuss the use of other blockchain frameworks for the protocol in Section \ref{sec::discussion}.

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{figures/fig_data_layer_worldState.pdf}
\caption{Cryptographic lock mechanism for off-state
}
\label{fig::Module2DataPlane} 
\end{figure}


\begin{table}
\centering
\caption{Summary of Main symbols.}
\begin{tabular}{l|l}
\hline
Symbol               & Description                                             \\ \hline
$F$                    & File to be transferred                             \\
$H(F)$                 & Hash of F                                           \\
$K_{aes}$            & Symmetric key        \\
$F_{enc}$            & File encrypted using $K_{aes}$                    \\
$H(F_{enc})$         & Hash of $F_{enc}$                                  \\
$K_{private}$        & Private key to sign $F_{enc}$ \\
$K_{public}$         & Public key to verify digital signature\\
$Signature(F_{enc})$ & Digital signature of $F_{enc}$                     \\ \hline
% $R$ & The result of digital signature verification                     \\\hline
\end{tabular}
\label{table::symbols}
\end{table}

\subsection{Stage 1: Preparing Off-State Data}

A data owner uploads big files to the off-state storage of her/his own blockchain node. The user also proposes a transaction---``Tx: file upload"---to record the profile of an uploaded file into the world state.
The file profile in the world state is public for searching.
%although how to perform search is out of scope of this paper. 
Fig. \ref{fig::Module2DataPlane} illustrates the \texttt{File Profile} entry in the world state, \texttt{ $\langle$file\_name, $H(F)$, owner, access\_rule, description$\rangle$}, where $H(F)$ is the hash of the file. $H(F)$ can be used to verify the integrity of a received file. 

\subsection{Stage 2: Sharing Off-State Data}
\label{Sharing_Off_State_Data}

Fig. \ref{fig::Module2} shows the workflow of sharing off-state data, e.g. a big file, in Fabric. It involves four transactions. These four transactions follow the same transaction lifecycle as introduced in Section \ref{subsubsec::FabricTransactionWorkflow}. However endorsers in each transaction can be different according to the specific endorsement policy setting. Fig. \ref{fig::Module2} shows which peers perform as endorsers to execute the chaincode in each transaction lifecycle.
% The receiver client first proposes a transaction to request the transfer agreement, then proposes a transaction to transfer the file from the sender node to the receiver node, next proposes a transaction to request the encryption key and at last proposes another transaction to query the encryption key and decrypt the received file. The details are as follows:

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{figures/fig_four_phases_fileShare.pdf}
\caption{Four phases in the off-state sharing protocol
}
\label{fig::Module2} 
\end{figure}

\subsubsection{Phase 1: File Transfer Request}
A user shall request the transfer of a particular file stored at the sender peer and the request shall pass the access control.
In Fabric, a user can propose a transaction to request a particular file, and the access control is governed by a specific endorsement policy. For example, the endorsement policy can be set as AND(Peer.Sender, Peer.Receiver), which stipulates both sender peer and receiver peer should agree on the file transfer.
An endorser checks if access rules in the corresponding \texttt{File Profile} are satisfied through smart contracts, and records the results in an \texttt{Event} entry of the world state. 
An \texttt{Event} entry is in the form of \texttt{ $\langle$event\_ID, flag, file\_name, sender, receiver$\rangle$} as shown in Fig. \ref{fig::Module2DataPlane}, where the $flag$ is a Boolean value indicating if the endorser permits the file transfer. 
According to the transaction workflow in Fabric introduced in Section \ref{subsubsec::FabricTransactionWorkflow}, when results (i.e. \texttt{Event} entry) returned from different endorsers are the same, the transaction can be generated, processed and recorded in a blockchain. The same \texttt{Event} entries mean the sender and receiver reach a consensus, either denial of or agreement on the file transfer. We call the corresponding transaction ``Tx: transfer request".

\subsubsection{Phase 2: Encrypted File Transfer}
After the file transfer request is approved, the user proposes another transaction---``Tx: file transfer"---to initiate the file transfer. In Fabric, the endorsement policy for ``Tx: file transfer" can be set as AND(Peer.Sender), which means only the sender peer works as an endorser.
The sender peer/endorser first checks $flag$ in the corresponding \texttt{Event} entry. The file transfer continues only if $flag$ is $True$.
%The sender can transfer a file in off-state through smart contracts.

The sender peer can then encrypt and sign the file, and send the encrypted file to the receiver peer via a file transfer protocol such as \textit{SFTP}. 
The receiver peer stores the encrypted file in its off-state storage.
In Fabric, the encryption key and related information of the encrypted file are put in the world state as an \texttt{Encryption Key} entry which is a PDC. PDC can guarantee that only PDC members can see the actual encryption key and others only know its hash. In this phase, only the sender peer is the PDC member. The \texttt{Encryption Key} entry is in the form of \texttt{$\langle$key\_ID, event\_ID $H(F_{enc})$, $K_{aes}$, $Signature(F_{enc})$, $K_{public}$ $\rangle$}, where $K_{aes}$ is the key to decrypt the encrypted file.
%It should one-to-one correspond to the \texttt{Event} entry for one-to-one correspondence between $K_{aes}$ and \texttt{Event}. 

%To establish the chain of custody, the sender encrypted the file and the receiver has to request the key through a transaction.
%In Fabric, a sender can transfer an encrypted file to a receiver, and store the corresponding encryption key as PDC in the world state. PDC can guarantee that only PDC members can see the actual encryption key and others only know its hash. If the receiver wants to decrypt the received encrypted file, she/he must request the encryption key in the world state through a transaction, which will be recorded in the blockchain. 


\subsubsection{Phase 3: Key Retrieval}
A user first checks if the receiver peer has received the transferred file. Only after the receiver peer has received the file does the user propose a transaction---``Tx: key access"---to request $K_{aes}$ from the sender peer to decrypt the encrypted file $F_{enc}$. Otherwise, the user does nothing. In Fabric, a user can send a query request to the receiver peer to check if $F_{enc}$ exists. The query request will not generate a transaction. Recall only the sender peer stores the original $K_{aes}$ and other nodes store the hash. The endorsement policy for ``Tx: key access" is set as AND(Peer.Sender) so that the sender peer performs as an endorser and adds the receiver peer to the PDC member list. Therefore, the receiver peer will be able to retrieve $K_{aes}$. 


\subsubsection{Phase 4: File Decryption}
Finally, the user proposes the last transaction ---``Tx: file decryption"---to query $K_{aes}$ to decrypt $F_{enc}$. In Fabric, the endorsement policy can be set as AND(Peer.Receiver) so that the receiver peer performs as an endorser, which can access $F_{enc}$ in its off-state storage using smart contract. The receiver peer first queries the \texttt{Encryption Key} entry in the world state for $K_{aes}$ and then decrypt $F_{enc}$.


\subsection{Security Analysis}
\label{sec::stage3}

%We design corresponding audit policies to solve disputes in big file sharing. The audit policies can be used to find out the dishonest participant by analysing the data in ledger, i.e. world state and blockchain. Ledgers provide anti-tampering proof. 
%Some authoritative arbitration institutions can involve in to conduct audit and punish the dishonest participant. 

We now show that the mechanisms in our off-state sharing protocol can ensure the integrity of chain of custody of the off-state data. That is, the user cannot deny that she/he has received the requested off-state data.
We assume the underlying blockchain infrastructure, i.e. all peers, is secure, and smart contracts execute as designed.
The assumption is reasonable since the peer administrators can adjust the user privilege to meet the need. \looseness=-1

An auditor can find out if a user has received a transferred file by searching for two transactions ``Tx: key access" and ``Tx: file decryption" related to the particular file from the blockchain. In our protocol, the receiver peer has to obtain $K_{aes}$ in order to decrypt the encrypted file $F_{enc}$, which the sender sends.
$K_{aes}$ is stored in the world state of the ledger, which guarantees the integrity of the data because of the underlying blockchain framework. When a user proposes the transaction ``Tx: key access", the receiver peer will receive $K_{aes}$. 
Once the receiver peer obtains $K_{aes}$, the user has to propose the transaction ``Tx: file decryption" to get decrypted file $F$. It can be observed that if the receiver peer does not receive $F_{enc}$, the user will not propose ``Tx: key access". If the receiver peer receives $F_{enc}$ but the user does not propose ``Tx: key access" to request $K_{aes}$, the receiver peer can not get the original file $F$.

An auditor can also find out if a sender peer has transferred a file by searching for ``Tx: file transfer" related to the particular file from the blockchain. In our protocol, ``Tx: file transfer" will trigger smart contracts to transfer a file in the off-state storage and stores \texttt{Encryption Key} in the world state. The integrity of ``Tx: file transfer" can be guaranteed by the underlying blockchain framework.

A user may wrongfully claim she/he receives a wrong file $f$. The transaction history maintained by the blockchain system actually provides proofs to dispute the claim. 
``Tx: file upload" and ``Tx: transfer request" can provide proofs to verify the integrity of the transferred file. In our protocol, a file owner records \texttt{File Profile} in the world state by proposing ``Tx: file upload". The sender peer and receiver peer should agree on a file sharing event which is recorded in the \texttt{Event} entry by ``Tx: transfer request". The file name in \texttt{Event} is related to a particular \texttt{File Profile}. ``Tx: transfer request" in blockchain can prove the sender and receiver peers have agreed on transferring a specific file and $H(F)$ in \texttt{File Profile} can be used to verify if $f$ matches with $H(F)$.
%If matched, $f$ is correct.



% Off-state data is managed by smart contracts and smart contracts retrieve and store the file profile information in the world state. The integrity of the file profile information can be ensured by the Smart contracts and underlying blockchain framework. The information in the world state can be used to verify the integrity of off-state data. $F$ or $F_{enc}$ can be verified through $H(F)$ and $H(F_{enc})$ in the world state. $F_{enc}$ is signed by the sender peer. The blockchain offers non-repudiation and the user's wrongful claim can be disputed. 
















==> CNS2021_File_sharing_arXiv/sections/sec6_evaluation.tex <==
\section{Evaluation}
\label{sec::Evaluations}

We have implemented a prototypical off-state sharing system, {\em BOSS}, based on Hyperledger Fabric, and evaluate its feasibility and performance in this section.

\subsection{Experiment Setup}
\label{sec::systemFramework}

Fig. \ref{fig::framework} shows the prototypical BOSS, which has three organizations, i.e. org1, org2 and org3. Org1 and org2 are the sender and the receiver, and each party contributes one peer node and one client (user/owner) node. Org3 is an auditing organization, and contributes one peer node and one orderer node. We implement our off-state sharing protocol using chaincode of Fabric and adopt \textit{SFTP} \cite{sftp_Wikipedia} to perform file transfer.

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{figures/fig_framwork.pdf}
\caption{Prototypical off-state sharing system (BOSS) based on Hyperledger Fabric
% \Fu{Font too small. Shall be similar to body text font size}
}
\label{fig::framework} 
\end{figure}

It can be observed that in our system, peer nodes are different from the conventional Fabric peer nodes. We integrate an off-state storage and the \textit{SFTP} service into peer nodes of interest. The chaincode can transfer and retrieve files from the local off-state storage. 

We implement the prototypical system and deploy it across three physical computers. Table \ref{table::setup} lists the configuration of the computers for sender, receiver and auditor nodes.
The sender computer and the receiver computer are located in different buildings on a university campus. All Fabric nodes run in Docker containers, which form the Fabric network. We use \textit{Golang} to develop the chaincode and use \textit{Node.js} to develop the client application that a user uses to propose transactions to the peer nodes.

\begin{table}[ht]
\centering
\caption{Blockchain Node Information in Prototypical BOSS}
\setlength{\tabcolsep}{0.3mm}{
\begin{tabular}{c|c|c|c|c|c}
\hline
Computer & Role                  & OS                                                 & Memory & Disk & CPU                                                                                            \\ \hline
1      & Sender   & \begin{tabular}[c]{@{}c@{}}Ubuntu\\ 18.04\end{tabular} & 64GB   & 1TB  & \begin{tabular}[c]{@{}c@{}}Intel Xeon(R) Gold\\ 6128 CPU@3.40GHz\\ ×24 Processor\end{tabular}  \\ \hline
2      & Receiver     & \begin{tabular}[c]{@{}c@{}}Ubuntu\\ 18.04\end{tabular} & 32GB   & 1TB  & \begin{tabular}[c]{@{}c@{}}Intel Core i7-6700\\ CPU@3.40GHz\\ × 8 Processor\end{tabular}       \\ \hline
3      & Auditor  & \begin{tabular}[c]{@{}c@{}}Ubuntu\\ 16.04\end{tabular} & 64GB   & 1TB  & \begin{tabular}[c]{@{}c@{}}Intel Xeon(R) Gold\\ 6128 CPU@3.40GHz\\ × 49 Processor\end{tabular} \\ \hline
\end{tabular}}
\label{table::setup}
\end{table}


\subsection{Performance and Feasibility}

We use \textit{Golang}'s \textit{SFTP} package to perform file transfer and find that the sender's buffer size parameter affects speed and latency of \textit{SFTP}. The latency refers to how long it takes to finish a particular operation. To find an optimal buffer size, we conduct \textit{SFTP} with different buffer sizes between two docker containers on physical Computer 1 and Computer 2 using a 576MB file and a 1.2GB file. Fig. \ref{fig::SFTP_buffer} shows how the buffer size affects the file transfer latency of \textit{SFTP}.
It can be observed that a buffer size of more than 1MB will not reduce the latency further. So we set the buffer size as 1MB in our system.

\begin{figure}[ht]
\centering
\includegraphics[width=1\columnwidth]{figures/fig_sftp_bufferSize_docker.pdf}
\caption{\textit{SFTP} latency versus buffer size
}
\label{fig::SFTP_buffer} 
\end{figure}

We use files of different types and various sizes to evaluate BOSS' feasibility and performance. Table \ref{table::file_list} lists those test files. Recall that a file sharing session involves four transactions as shown in Fig. \ref{fig::Module2}. We evaluate the latency of different transactions and the latency of the whole session. We evaluate how the file size and the parallel file transfers affect the latency. 

\begin{table}[h]
\centering
\caption{Test File List}
\begin{tabular}{lll}
\hline
Type & Size  & Describtion                       \\ \hline
.pdf & 67MB  & ``C++ Primer Plus" eBook          \\
.mp4 & 218MB & An over 5 hours song list video   \\
.tif & 576MB & The image of Moon from NASA       \\
.zip & 1.2GB & A collection of medical images    \\
.rar & 2.6GB & The compressed file of one movie  \\
.zip & 5.3GB & The compressed file of two movies \\ \hline
\end{tabular}
\label{table::file_list}
\end{table}

\begin{figure*}[!ht]
\begin{minipage}[c]{0.65\columnwidth}
\centering
\includegraphics[height=0.72\textwidth]{figures/fig_transfer_request&key_access.pdf}
\caption{Transaction latency of ``Tx: transfer request" and ``Tx: key access"}
\label{fig::1par_req} 
\end{minipage}
\hspace{0.3cm}
\begin{minipage}[c]{0.65\columnwidth}
\centering
\includegraphics[height=0.72\textwidth]{figures/fig_trans_sftp_decrypt.pdf}
\caption{SFTP latency and transaction Latency of ``Tx: file transfer" and ``Tx: file decryption"}
\label{fig::1par_tran_dec}
\end{minipage}
\hspace{0.3cm}
\begin{minipage}[c]{0.65\columnwidth}
\centering
\includegraphics[height=0.72\textwidth]{figures/fig_wholeLatency_1par.pdf}
\caption{File sharing session latency}
\label{fig::1par_whole}
\end{minipage}
\end{figure*} 


\begin{figure*}[!ht]
\begin{minipage}[c]{0.65\columnwidth}
\centering
\includegraphics[height=0.64\textwidth]{figures/fig_requestAgree_latency_mulPar_all.pdf}
\caption{Transaction latency of ``Tx: transfer request" in different parallel transfer cases}
\label{fig::mul_par_requestAgree_Tx} 
\end{minipage}
\hspace{0.3cm}
\begin{minipage}[c]{0.65\columnwidth}
\centering
\includegraphics[height=0.64\textwidth]{figures/fig_requestKey_latency_mulPar_all.pdf}
\caption{Transaction latency of ``Tx: key access" in different parallel transfer cases}
\label{fig::mul_par_requestKey_Tx} 
\end{minipage}
\hspace{0.3cm}
\begin{minipage}[c]{0.65\columnwidth}
\centering
\includegraphics[height=0.64\textwidth]{figures/fig_transfer_latency_mulPar_all.pdf}
\caption{Transaction latency of ``Tx: file transfer" in different parallel transfer cases}
\label{fig::mul_par_transfer_Tx}
\end{minipage}
% \hspace{0.3cm}
\end{figure*} 


\begin{figure*}[!ht]
\begin{minipage}[c]{0.65\columnwidth}
\centering
\includegraphics[height=0.64\textwidth]{figures/fig_sftp_latency_mulPar_all.pdf}
\caption{SFTP latency in different parallel transfer cases}
\label{fig::mul_par_sftp} 
\end{minipage}
\hspace{0.3cm}
\begin{minipage}[c]{0.65\columnwidth}
\centering
\includegraphics[height=0.64\textwidth]{figures/fig_decrypt_latency_MulPar_all.pdf}
\caption{Transaction latency of ``Tx: file decryption" in different parallel transfer cases}
\label{fig::mul_par_decrypt_Tx} 
\end{minipage}
\hspace{0.3cm}
\begin{minipage}[c]{0.65\columnwidth}
\centering
\includegraphics[height=0.68\textwidth]{figures/fig_whole_latency_all_par.pdf}
\caption{Average file sharing session latency in different parallel transfer cases}
\label{fig::mul_par_ave_event} 
\end{minipage}
\hspace{0.3cm}
\end{figure*} 

\begin{table}
\centering
\caption{Percentage of SFTP Latency in ``Tx: file transfer" Latency}
\begin{tabular}{c|cccc}
\hline
Size                       & 1 Parallel & 2 Parallel & 4 Parallel & 8 Parallel \\ \hline
\multicolumn{1}{c|}{67MB}  & 75.30\%    & 85.33\%    & 93.38\%    & 92.01\%    \\
\multicolumn{1}{c|}{218MB} & 88.05\%    & 92.82\%    & 95.73\%    & 84.13\%    \\
\multicolumn{1}{c|}{576MB} & 92.43\%    & 94.86\%    & 87.50\%    & 82.33\%    \\
\multicolumn{1}{c|}{1.2GB} & 91.18\%    & 85.13\%    & 83.86\%    & 83.71\%    \\
\multicolumn{1}{c|}{2.6GB} & 86.24\%    & 85.71\%    & 84.36\%    & 84.08\%    \\
\multicolumn{1}{c|}{5.3GB} & 85.84\%    & 83.56\%    & 81.39\%    & 82.68\%    \\ \hline
\end{tabular}
\label{table::sftpPercentTran}
\end{table}

\subsubsection{\textbf{File Size}}
\label{sec::file_size_eva}

For each file in Table \ref{table::file_list}, we conduct the file transfer 32 times. Each time only one file transfer is performed. The results are shown in Figs. \ref{fig::1par_req}--\ref{fig::1par_whole}.
% , Fig.\ref{fig::1par_tran_dec} and Fig.\ref{fig::1par_whole}.

Fig. \ref{fig::1par_req} shows the latency of ``Tx: transfer request" and ``Tx: key access" across different file sizes. It can be observed that the latency of these two transactions are relatively stable and the file size has minor affect on the latency. This is reasonable since these two transactions only operate on the world state data.

Fig. \ref{fig::1par_tran_dec} shows the latency of ``Tx: file transfer" and ``Tx: file decryption". It can be observed that the latency of these two transactions rapidly increase as the file size increases.
%the file size has considerable affect on the latency. 
The reason is ``Tx: file transfer" involves multiple cryptographic calculations to encrypt files and uses \textit{SFTP} to transfer the file. 
%Therefore, it is reasonable that its latency is affected by the file size. 
Fig. \ref{fig::1par_tran_dec} shows the latency of the \textit{SFTP} transmission. Table \ref{table::sftpPercentTran} shows the percentage of the \textit{SFTP} latency in the ``Tx: file transfer" latency. It can be observed that the \textit{SFTP} latency accounts for a large proportion of the whole ``Tx: file transfer" latency.  ``Tx: file decryption" involves multiple cryptographic calculation to decrypt the file. So it is reasonable that its latency is affected by the file size.

Fig. \ref{fig::1par_whole} shows the average latency of one file sharing session. It can be observed that the latency of one file sharing session rapidly increases as the file size increases. It is reasonable because normally more time is needed to transfer larger files.

\subsubsection{\textbf{Parallel Transfer}}
\label{sec::par_eva}

We also want to find out if we can transfer multiple files in parallel between two nodes and evaluate the performance.   
%further evaluate the latency in different parallel file transfer cases. 
In our experiments, for each file, the number of simultaneous parallel file transfer sessions is 1, 2, 4 and 8, denoted as 1-P, 2-P, 4-P and 8-P in Figs. \ref{fig::mul_par_requestAgree_Tx}--\ref{fig::mul_par_ave_event}, which show the experiment results.
In each case, the file is transferred 32 times in total. For example, in the case of 4-P (4 parallel file transfer session), we perform the experiments 8 times and the file is transferred 32 times ($4\times8$).
%\red{For each file, we conduct the file sharing event 32 times in total. We in parallel propose different number of file sharing events at the same time. For example, we in parallel propose 4 file transfer events for 8 rounds. The results are shown in Fig.\ref{fig::mul_par_requestAgree_Tx}-\ref{fig::mul_par_ave_event}. }

We make the following observations. As the number of parallel sessions increases, the latency of ``Tx: transfer request" and ``Tx: key access" is relatively stable as shown in Fig. \ref{fig::mul_par_requestAgree_Tx} and Fig. \ref{fig::mul_par_requestKey_Tx}. However the latency of ``Tx: file transfer" and ``Tx: file decryption" increases as the number of parallel sessions increases. Fig. \ref{fig::mul_par_sftp} further shows the latency of \textit{SFTP} involved in ``Tx: file transfer" in different parallel transfer cases. Table \ref{table::sftpPercentTran} shows the percentage of \textit{SFTP} incurred latency in the ``Tx: file transfer" latency. It shows the same trend as ``Tx: file transfer" and accounts for the most of the transaction latency. \looseness=-1

Fig. \ref{fig::mul_par_ave_event} shows the average latency of one file sharing session in different parallel transfer cases. It can be observed that the average file transfer session latency increases as the number of parallel transfer sessions increases. This is reasonable because simultaneous parallel file transfer sessions share the network bandwidth. More sessions mean less network bandwidth for each file transfer session.
% For each file size, the average latency is calculated by Formula (\ref{eqn::ave_event_latency}), 
% \begin{eqnarray}
% \overline{Latency(n)} = T_{n}/{n},
% \label{eqn::ave_event_latency}
% \end{eqnarray}
% where $n$ is the number of parallel sessions and $T_n$ is the whole time to transfer $n$ files in parallel. 




% \subsection{Timeout Discussion}

%that when the file becomes larger, does not decreases as the parallel number increases. This indicates that the concurrency capability of Hyperledger Fabric nodes is not ideal. When there are too many high-latency transactions to handle, it becomes unstable.

% \subsubsection{Throughput}

% \subsection{Optimization through Load Balance}

% The evaluation results in terms of parallel are not ideal as analyzed in Section \ref{sec::par_eva}. We propose a load balance scheme to optimize the latency in parallel cases. As shown in Fig.\ref{fig::framework}, both the sender and the receiver contribute only one node. Based on the results in Section \ref{sec::par_eva}, the capability of Hyperledger Fabric nodes is unsatisfactory to handle multiple long-time transactions in the same time. To mitigate this, we propose to increase the nodes belong to each party, and evenly distribute the parallel file transfer events to different nodes.

% To demonstrate the efficiency of the load balance scheme, we use the system architecture as shown in Fig.\ref{fig::load_balance} to re-conduct the parallel experiments. The sender contributes four peer nodes and the receivers contribute two peer nodes. All nodes still run in Docker containers. The results are shown in Fig.\ref{fig::mul_par_event_opt}. Comparing with Fig.\ref{fig::mul_par_event}, the average latency of one event is optimized in all parallel cases. It is reasonable to get a better system performance when more resources are contributed.

==> CNS2021_File_sharing_arXiv/sections/sec7_discussion.tex <==
\section{Discussion}
\label{sec::discussion}

In this section, we discuss the impact of chaincode execution timeout on big file sharing, potential implementation of BOSS with other blockchain frameworks, difference between off-state and off-chain and out-of-band distribution of received files by users. \looseness=-1

\subsection{Chaincode Execution Timeout}

% Current blockchain frameworks are not specifically designed to manage large data and high-latency transactions. 
% We summarize the problems in evaluation experiments, which indicates future improvements for the blockchain framework used to build the large file sharing system.

In Fabric, chaincode has a system wide execution timeout setting. The default timeout value is $30s$. In BOSS, the chaincode invokes SFTP for file transfer and waits for SFTP to finish. 
However, $30s$ is far from enough for transferring a big file and the chaincode will time out.
This timeout setting can be changed in the docker configuration file of Fabric, but cannot be changed at runtime based on the size of the file.
We find setting the timeout to infinity does not work in Fabric either and plan to revise Fabric as future work so that we can change the timeout flexibly.

\subsection{Implementation based on Other Blockchain Frameworks}

Bitcoin is not appropriate to implement BOSS. First, Bitcoin is a permissionless blockchain system. It is hard to implement access control. Second, Bitcoin essentially is a blockchain-based cryptocurrency application. There is no existing mechanism like smart contracts for programming. It will be a challenge and tedious to develop other applications over it.

Enterprise Ethereum \cite{enterpriseEthereum} can be used to implement a blockchain off-state sharing system.
Enterprise Ethereum \cite{Hyperledger_Besu}\cite{goquorum} is a permissioned blockchain framework for enterprise applications. It has many similar features to Fabric.
First, there is a private world state as well as a public world state for each enterprise Ethereum node. The private world state is only shared within a private group.
Enterprise Ethereum provides a private transaction manager, which can be used to keep transactions private among a private group. 
The private world state is similar to PDC in Fabric and can be used to manage the encryption key access required by BOSS.
Second, there is a private contract mechanism. A private contract is only available and executed on a subset of nodes. This is actually similar to customizable chaincode in Fabric and is flexible for the sender/receiver peers to implement their own business logic.
Third, the language of smart contracts is Solidity \cite{solidity_Wikipedia} in Ethereum. Solidity is a Turing-complete program language which can be used to implement a business logic. 

\subsection{Difference between Off-State and Off-Chain}

Off-state is different from off-chain \cite{poon2016bitcoin,coleman2018counterfactual,dziembowski2018general}, and existing off-chain protocols can not be utilized to ensure the safety of off-state data. 
The off-chain technique is designed to scale the blockchain systems and improve transaction throughput. 
It constructs transactions off-chains, and submits one transaction containing the final results to update the world state.
Essentially, the off-chain protocol is designed to guarantee the safety of the world state. 
The well-known off-chain technique is the payment channel in Bitcoin \cite{poon2016bitcoin}. A payment channel first locks some on-chain cryptocurrencies, i.e. the UTXOs state. Then it constructs transaction off-chains to conduct micropayments using locked cryptocurrencies, but does not commit these transactions involving micropayments to the blockchain. At last, it commits one transaction that represents final micropayment results to the main blockchain to update the UTXOs world state.
Off-chain can not solve the storage limitation issues or be used for big file sharing. 

\subsection{Out-of-band Data Distribution}

Once the file is transferred to a user through BOSS, the user may stealthily send the file to other parties through out-of-band commnunication but not through BOSS. It will be hard to trace those files. This is a generic problem in data sharing, not specific to our system. Potential solutions include digital watermark \cite{van1994digital} and traitor tracing \cite{boneh1999efficient}, which adds some additional information to the files. Another strategy will be to limit the user capabilities with the files to particular workstations and use physical security and particular configurations that allow file transfer only through BOSS.
%This is out of scope of this paper and we mainly focus on safety of file sharing process.




==> CNS2021_File_sharing_arXiv/sections/sec8_relatedwork.tex <==
\section{Related Work}
\label{sec::related_work}

Related work on blockchain-based data sharing systems does not focus on the big file sharing. It does not address the specific challenges in big file sharing or solve the problem.

\subsection{Data Sharing in Ledgers}
In most existing blockchain-based data sharing systems, shared data is stored in ledgers. Users set or get shared data through proposing transactions to the blockchain system. Transactions are the carriers of the shared data. 
Wang et al.\cite{wang2020blockchain} utilize the blockchain system as the back end to transmit and store data from the front-end wireless body area networks (WBAN). All blockchain nodes maintain the same data and all participants such as doctors and insurance providers share the same WBAN data.
Zhang et al. \cite{zhang2018towards} propose a blockchain-based secure and privacy-preserving personal health information (PHI) sharing scheme. The original PHI records are stored in the ledger of the private blockchain of each hospital, and the consortium blockchain keeps records of the indexes of the PHI. 
Jiang et al. \cite{jiang2018blochie} propose a blockchain-based platform for healthcare information exchange. They use two loosely coupled blockchains to handle different kinds of healthcare data, including highly sensitive electronic medical records (EMRs) and personal healthcare data (PHD). 
These existing schemes are not suitable for big file sharing applications because big files cannot be stored in blockchain ledgers due to the storage limitation as analyzed in Section \ref{sec::Storage_Limitations}.


\subsection{Data Sharing Outside Ledgers}
There are systems that store shared data outside the ledgers in blockchain systems. 
Xia et al. \cite{xia2017medshare} propose a blockchain-based solution to sharing medical data among cloud service providers. In their design, smart contracts retrieve requested data from existing database infrastructure, outside of a blockchain system. The retrieved results are recorded in the blockchain. It is impractical to record big files in a blockchain. 
Lu et al. \cite{lu2019blockchain} design a blockchain empowered privacy-preserved data sharing architecture for industrial IoT. They exploit the privacy-preserved federated learning algorithm to learn the data model and share the data model instead of revealing the actual data. They use the blockchain to retrieve and manage the accessibility of data.
Zhang et al. \cite{zhang2018fhirchain} choose to store and exchange only reference pointers of the sensitive data in the blockchain. A data requester should first get a token from the blockchain system and then use the token to access original data in the database outside the blockchain. 

These existing schemes do not focus on big file sharing. They also fail to consider security requirements such as dealing with dishonest users, and fail to design a protocol for secure off-state sharing.
Wang et al. \cite{PDCFabric} find misuse of PDC in Fabric may endanger a blockchain system and BOSS avoids such issues in the implementation.

% design a specific protocol to guarantee the safety of large files transfer between trustless parties considering dishonest participants.







==> CNS2021_File_sharing_arXiv/sections/sec9_conclusion.tex <==
\section{Conclusion}
\label{sec::Conclusion}

In this paper, we solve a novel problem---how to securely share big data files within a blockchain system and establish the chain of custody of the shared data.
Such a data sharing application is critical for protecting intellectual property (IP) theft and fighting industrial espionage in fields including biomedical research.
We denote data such as big files stored at a blockchain node but outside of the ledger as off-state.
Three challenges including storage space limitation, privacy requirement and security requirement are discovered in implementing a blockchain off-state sharing system (BOSS).
We carefully present our off-state sharing protocol. The transactions generated by our protocol will serve as auditing evidence for the chain of custody.
We implement BOSS over Hyperledger Fabric and conduct extensive experiments to evaluate the feasibility and performance of BOSS.
%using files of different types and various size. We measure the latency of different transactions and the latency of the whole file sharing session, and analyze how the file size and the parallel file transfers affect the latency. 

% which can establish the chain of custody of the big data files.


==> CNS2021_File_sharing_arXiv/sections/trash/sec4.tex <==
\delete{
\subsubsection{Scenario 1: A receiver denies that it has received a transferred file}

In our four-phase file sharing protocol, the receiver has to obtain $K_{aes}$ in order to decrypt the encrypted file $F_{enc}$, which the sender sends.
%the receiver should get the access permission of $K_{aes}$ and then query $K_{aes}$ to decrypt $F_{enc}$ to get $F$.
$K_{aes}$ is stored in the world state of the ledger, which guarantees its integrity because of the underlying blockchain framework. That is, once a receiver proposes ``Tx: key access", the receiver will definitely receive $K_{aes}$. The user can then propose ``Tx: file decryption" to get $F$. In this scenario, the auditor can find out the fact by retrieving ``Tx: key access" in the blockchain. If the receiver receives $F_{enc}$ but does not propose a transaction to request $K_{aes}$, the receiver can not get the original file $F$. In this situation, we regard it as the receiver does not receive the file $F$. 


\subsubsection{Scenario 1: Dishonest Sender}
As discussed in \textit{Challenge 3---Security Requirement}, the sender may wrongly declare that she/he has transferred the file but actually not.
%We define the policy to identify if the sender has transferred the file as follows.

%Once the \texttt{Encryption Key} entry is recorded in the world state, it means the sender claims that she/he has transferred the file.
%\textit{Security Analysis:} 
In our four-phase file sharing protocol, an \texttt{Encryption Key} entry will be recorded in the world state while the sender transfers the encrypted file to the receiver. The world state is always updated through transactions. The corresponding transaction ``Tx: transfer file" is recorded in an immutable blockchain. 
%Auditors can find out the fact by retrieving the corresponding transaction in the blockchain. 
If the sender only sets the \texttt{Encryption Key} entry but does not send the encrypted file, the receiver will not request the encryption key since she/he does not receive any encrypted file. The file sharing process will not be completed.
It can not benefit the sender. Therefore, the sender has no incentive to only set the encryption key to claim he has sent the file but not actually sends $F_{enc}$. 


\subsubsection{Scenario 3: Wrong Files}
In \textit{Challenge 3---Security Requirement}, a receiver may transfer a wrong file. The receiver may claim that the received file is not the desired one. We define the policy to identify if the transferred file is consistent with \texttt{File Profile} in world state as follows:

% The receiver may claim that the received file is not the desired one. We define the policy to identify if the transferred file is consistent with the file profile in the world state as following: 

\textbf{Policy 3. File Correctness:} The receiver provides the received encrypted file $F_{enc}$ and \texttt{Encryption Key} in world state to an auditor. Auditor can check if the \texttt{Encryption Key} match the PDC hash in the auditor node's world state who is a PDC non-member. If the \texttt{Encryption Key} is the correct one, an auditor can judge the file correctness according to the following three conditions: 
\begin{enumerate}
 
\item[i)] $F_{enc}$ can pass the signature verification as show in formula (\ref{eqn::verify_rsa}). That is the $R$ is $True$.
\begin{eqnarray}
R = Verify(Signature(F_{enc}), H(F_{enc}), K_{public})
\label{eqn::verify_rsa}
\end{eqnarray}

\item[ii)] $F_{enc}$ match the $H(F_{enc})$ in \texttt{Encryption Key};

\item[iii)] The plaintext $F$ decrypted from $F_{enc}$ matches $H(F)$ in \texttt{File Profile} recorded in world state. 
\end{enumerate}
If any one condition is violated, the transferred file is incorrect. If all conditions are satisfied, the transferred file is correct.

\textit{Security Analysis:} 
The information used to audit includes $F_{enc}$ and some data in world state. $F_{enc}$ is in off-state but can be verified through $H(F_{enc})$ in world state. Data in world state is safe and verifiable. 
An auditor can identify who perform dishonestly so as to ascribe blame.
If condition i) is violated, it means the receiver provides wrong information to the auditor. 
If condition i) is satisfied but condition ii) is violated, it means that the sender sends wrong $F_{enc}$ that does not match $H(F_{enc})$ in the world state.
If condition iii) is violated and condition i) and ii) are satisfied, it means the sender sends wrong file that does not match the file profile in the world state. 

In the case of that both participants behave honestly but the receiver is unsatisfied with the file content, the issue should be solved by authoritative arbitration institution and the blockchain system only provides proof.

% \subsection{Apply Traitor Tracing and Water Markers Techniques}

}

==> CNS2021_File_sharing_arXiv/sections/trash/sec5_system.tex <==
\section{Proof-of-Concept Implementation Based on Hyperledger Fabric}
\label{sec::poc_system}

\Fu{Can we use Etherum and Bitcoin to implement this system? May need to merge this section into last section}
%This section presents details of the proof of concept (PoC) implementation of the system.
We design a prototypical big file sharing system based on Hyperledger Fabric.
%We first briefly present features of Hyperledger Fabric that fit our big files sharing mechanism. 
Then we introduce the PoC system framework, workflow and some implementation details.

% Hyperledger Fabric is a popular permissioned blockchain framework, which only authorized participants can involve in.

\subsection{System Framework and Workflow}
\label{sec::systemFramework}

Framework of the PoC system is shown in Fig. \ref{fig::framework}. Three organizations, i.e. org1, org2 and org3, cooperatively build this system. Org1 and org2 respectively represent the sender and the receiver, and each party contributes one peer node and one client node. Org3 represent an auditor organization, and contribute one peer node and one orderer node. Smart contract is also called chaincode in Fabric. We implement our off-state integration mechanism using chaincode, and adopt \textit{SFTP} \cite{sftp_Wikipedia} to conduct file transfer.

\subsubsection{Peer Modifications}
In our system, peer nodes are different from the traditional Hyperledger Fabric peer nodes. We integrate an off-state and the \textit{SFTP} service to some peer nodes. We create an off-state storage space in the chaincode's workspace. So the chaincode can interact with the local off-state and operate on it. Nodes in Hyperledger Fabric run in Docker containers\cite{anderson2015docker} without \textit{SFTP} service. We install \textit{SFTP} service \cite{sftp_Wikipedia} in some peer nodes. 
% In Hyperledger Fabric, chaincode is a program written by general-purpose programming languages, which usually have \textit{SFTP} service library. 
So file owners can upload files to off-state, and the chaincode can invoke \textit{SFTP} to transfer files in local off-state.

\subsubsection{Transaction Workflow}

%In Hyperledger Fabric, as shown in Fig.\ref{fig::framework}, a common transaction workflow is as follows: 1. A client proposes a transaction proposal to some peer nodes, i.e. endorsers, specified by the endorsement policy; 2. Endorsers execute the chaincode, sign the execution results, and return the results with corresponding signatures to the client as proposal responses; 3. If the returned execution results from different endorsers are the same, the client assembles a transaction and sends it to the orderer node. 4. The orderer node collects multiple transactions in the same time, bundles transactions into a new block, and distribute the new block to all peers including both endorsers and non-endorsers. 5. All peers validate the transactions in the received new block. If the transaction is valid, the peer will update world state according to execution results. After validating all transactions, each peer appends the new block to a blockchain. 

In our three-phase file sharing event, one event involves four transactions as shown in Fig. \ref{fig::Module2}. All involved transactions follow the same common transaction workflow. The only difference is that endorsers are different in Steps 1 and 2. according to different endorsement policy setting. 


\subsection{Endorsement Policy Setting}
\label{sec::Endorsement_Policy_Set}

We illustrate the endorsement policy setting for involved four transactions in one file sharing event, including ``Tx: request permission", ``Tx: transfer file", ``Tx: request key" and ``Tx: decrypt file". The default chaincode-level endorsement policy is set as AND(Org1MSP, Org2MSP), which means peer nodes from both org1 and org2 need endorse a transaction. Note that org3 does not involve in any endorsing and only synchronizes the ledger data, i.e. world state and blockchain. In the following illustration, we assume Peer1 is the sender and Peer2 is the receiver.

% \subsubsection{File Uploading Event}
% In Module 1, when add a new file to the off-state, the smart contract should record the File Profile entry to the world state. The corresponding entry is $\langle$file\_name, $H(F)$, owner, access\_rule, description$\rangle$. The smart contract should read the file from the off-state and calculate the file hash. Since peer nodes only maintains their own files, only the file's owner peer can get the hash information. So the key-level policy for this entry should be customized. For example, when the user add file 1 to the Peer 1, the key-level policy for file 1 profile entry should be AND(Org1MSP), which mean only Peer 1 acts as the endorser and execute the smart contract. Though other peer nodes do not execute the smart contract, they will also store the entry in the world state and store the corresponding transaction in the blockchain. 

% \subsubsection{Module 2 implementation}
% Transferring files involves three phases:

\subsubsection{Tx: request permission}
During this transaction, chaincode verifies if pre-defined access control rules are satisfied, and records the verification result in an \texttt{Event} entry. This should be conducted by both sender and receiver, i.e. Peer1 and Peer2. So the endorsement policy for this transaction uses the default chaincode-level endorsement policy, i.e. AND(Org1MSP, Org2MSP). 

\subsubsection{Tx: file transfer}
During this transaction, chaincode conducts encrypting file, transferring file and writing \texttt{Encryption Key} to world state. $K_{aes}$ in \texttt{Encryption Key} should be kept only by the sender and other peers only store the hash. So \texttt{Encryption Key} should be set as a PDC and only the sender node Peer1 is the PDC member. Besides, only Peer1 owns the file to be encrypted and transfered. So the endorsement policy for this transaction should be customized as a collection-level policy and the policy should be AND(Org1MSP). That's only Peer1 performs as an endorser.

\subsubsection{Tx: request key}
During this transaction, chaincode should reset the PDC member of \texttt{Encryption Key} and add the receiver Peer2 to the PDC member. Then the receiver will own the original $K_{aes}$. The sender Peer1 should act as the endorser since it is the only original member of \texttt{Encryption Key}. The endorsement policy for this transaction should be AND(Org1MSP).

\subsubsection{Tx: query key and decrypt}
During this transaction, chaincode queries \texttt{Encryption Key} in world state to decrypt the encrypted file in the off-state. It is the receiver Peer2 who needs to decrypt the received encrypted file. And Peer2 now owns $K_{aes}$. So the endorsement policy for this transaction should be set as AND(Org2MSP).

% \subsubsection{Stage 3 implementation}

% If some disputes occur, the auditer organization will involved. The audit organizaton does not involve in the file uploading and file transferring. It only records all entries in its world state and all transactions in its blockchain. The auditer peer only conducts audit. So the smart contract running in the Peer 3 is different from Peer 1 and Peer 2. This can be implemented due to the customizable smart contracts feature in Hyperledger Fabric. According to the three audit policies in Section \ref{sec::stage3}, the smart contract needs query the file profile entry, encryption key entry and the transaction history. All these information locates in the auditer peer node, so the endorsement policy can be set as AND(Org3MSP).

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{figures/fig_framwork.pdf}
\caption{Framework of big files sharing system based on Hyperledger Fabric
\Fu{Font too small. Shall be similar to body text font size}}
\label{fig::framework} 
\end{figure}

% \subsection{Big Files Sharing Workflow}

%The whole file transfer process involves multiple transactions. At stage 1, the client proposes a transaction to record the new file uploaded to the off-state. 
%At stage 2, the receiver's client first proposes a transaction to request the transfer agreement. Then the sender's client proposes a transaction to transfer the file from one node to the other node. Next the receiver's client proposes a transaction to request the encryption key and at last proposes another transaction to query the encryption key and decrypt the received file. 
%At stage 3, the client can propose a transaction to conduct one policy check according to different scenarios.



%All involved transactions in the whole file transfer process follow the same common transaction workflow in Hyperledger Fabric. The only difference is that the corresponding endorsement policy involved in different transactions are different since these transactions operate different entries in the world state. We have analysed the endorsement policy setting for different entries in the last Section \ref{sec::systemFramework}. The common transaction workflow is as following: i) The client proposes a transaction proposal to the endorsers defined by the endorsement policy; ii) Endorsers execute the smart contract, sign the execution results, and return the results with corresponding signatures to the client; iii) If the returned results from different endorsers are the same, the client assembles a transaction and sends it to the orderer node. iv) The orderer node collects multiple transactions in the same time, blindly bundles transactions into new blocks, and distribute the new block to all peers including both endorsers and non-endorsers. v) All peers validate the transactions in the received new block. If the transaction is valid, the peer will update the data in the world state and append the new block to the blockchain. 

==> sections/trash/sec4.tex <==
\delete{
\subsubsection{Scenario 1: A receiver denies that it has received a transferred file}

In our four-phase file sharing protocol, the receiver has to obtain $K_{aes}$ in order to decrypt the encrypted file $F_{enc}$, which the sender sends.
%the receiver should get the access permission of $K_{aes}$ and then query $K_{aes}$ to decrypt $F_{enc}$ to get $F$.
$K_{aes}$ is stored in the world state of the ledger, which guarantees its integrity because of the underlying blockchain framework. That is, once a receiver proposes ``Tx: key access", the receiver will definitely receive $K_{aes}$. The user can then propose ``Tx: file decryption" to get $F$. In this scenario, the auditor can find out the fact by retrieving ``Tx: key access" in the blockchain. If the receiver receives $F_{enc}$ but does not propose a transaction to request $K_{aes}$, the receiver can not get the original file $F$. In this situation, we regard it as the receiver does not receive the file $F$. 


\subsubsection{Scenario 1: Dishonest Sender}
As discussed in \textit{Challenge 3---Security Requirement}, the sender may wrongly declare that she/he has transferred the file but actually not.
%We define the policy to identify if the sender has transferred the file as follows.

%Once the \texttt{Encryption Key} entry is recorded in the world state, it means the sender claims that she/he has transferred the file.
%\textit{Security Analysis:} 
In our four-phase file sharing protocol, an \texttt{Encryption Key} entry will be recorded in the world state while the sender transfers the encrypted file to the receiver. The world state is always updated through transactions. The corresponding transaction ``Tx: transfer file" is recorded in an immutable blockchain. 
%Auditors can find out the fact by retrieving the corresponding transaction in the blockchain. 
If the sender only sets the \texttt{Encryption Key} entry but does not send the encrypted file, the receiver will not request the encryption key since she/he does not receive any encrypted file. The file sharing process will not be completed.
It can not benefit the sender. Therefore, the sender has no incentive to only set the encryption key to claim he has sent the file but not actually sends $F_{enc}$. 


\subsubsection{Scenario 3: Wrong Files}
In \textit{Challenge 3---Security Requirement}, a receiver may transfer a wrong file. The receiver may claim that the received file is not the desired one. We define the policy to identify if the transferred file is consistent with \texttt{File Profile} in world state as follows:

% The receiver may claim that the received file is not the desired one. We define the policy to identify if the transferred file is consistent with the file profile in the world state as following: 

\textbf{Policy 3. File Correctness:} The receiver provides the received encrypted file $F_{enc}$ and \texttt{Encryption Key} in world state to an auditor. Auditor can check if the \texttt{Encryption Key} match the PDC hash in the auditor node's world state who is a PDC non-member. If the \texttt{Encryption Key} is the correct one, an auditor can judge the file correctness according to the following three conditions: 
\begin{enumerate}
 
\item[i)] $F_{enc}$ can pass the signature verification as show in formula (\ref{eqn::verify_rsa}). That is the $R$ is $True$.
\begin{eqnarray}
R = Verify(Signature(F_{enc}), H(F_{enc}), K_{public})
\label{eqn::verify_rsa}
\end{eqnarray}

\item[ii)] $F_{enc}$ match the $H(F_{enc})$ in \texttt{Encryption Key};

\item[iii)] The plaintext $F$ decrypted from $F_{enc}$ matches $H(F)$ in \texttt{File Profile} recorded in world state. 
\end{enumerate}
If any one condition is violated, the transferred file is incorrect. If all conditions are satisfied, the transferred file is correct.

\textit{Security Analysis:} 
The information used to audit includes $F_{enc}$ and some data in world state. $F_{enc}$ is in off-state but can be verified through $H(F_{enc})$ in world state. Data in world state is safe and verifiable. 
An auditor can identify who perform dishonestly so as to ascribe blame.
If condition i) is violated, it means the receiver provides wrong information to the auditor. 
If condition i) is satisfied but condition ii) is violated, it means that the sender sends wrong $F_{enc}$ that does not match $H(F_{enc})$ in the world state.
If condition iii) is violated and condition i) and ii) are satisfied, it means the sender sends wrong file that does not match the file profile in the world state. 

In the case of that both participants behave honestly but the receiver is unsatisfied with the file content, the issue should be solved by authoritative arbitration institution and the blockchain system only provides proof.

% \subsection{Apply Traitor Tracing and Water Markers Techniques}

}

==> sections/trash/sec5_system.tex <==
\section{Proof-of-Concept Implementation Based on Hyperledger Fabric}
\label{sec::poc_system}

\Fu{Can we use Etherum and Bitcoin to implement this system? May need to merge this section into last section}
%This section presents details of the proof of concept (PoC) implementation of the system.
We design a prototypical big file sharing system based on Hyperledger Fabric.
%We first briefly present features of Hyperledger Fabric that fit our big files sharing mechanism. 
Then we introduce the PoC system framework, workflow and some implementation details.

% Hyperledger Fabric is a popular permissioned blockchain framework, which only authorized participants can involve in.

\subsection{System Framework and Workflow}
\label{sec::systemFramework}

Framework of the PoC system is shown in Fig. \ref{fig::framework}. Three organizations, i.e. org1, org2 and org3, cooperatively build this system. Org1 and org2 respectively represent the sender and the receiver, and each party contributes one peer node and one client node. Org3 represent an auditor organization, and contribute one peer node and one orderer node. Smart contract is also called chaincode in Fabric. We implement our off-state integration mechanism using chaincode, and adopt \textit{SFTP} \cite{sftp_Wikipedia} to conduct file transfer.

\subsubsection{Peer Modifications}
In our system, peer nodes are different from the traditional Hyperledger Fabric peer nodes. We integrate an off-state and the \textit{SFTP} service to some peer nodes. We create an off-state storage space in the chaincode's workspace. So the chaincode can interact with the local off-state and operate on it. Nodes in Hyperledger Fabric run in Docker containers\cite{anderson2015docker} without \textit{SFTP} service. We install \textit{SFTP} service \cite{sftp_Wikipedia} in some peer nodes. 
% In Hyperledger Fabric, chaincode is a program written by general-purpose programming languages, which usually have \textit{SFTP} service library. 
So file owners can upload files to off-state, and the chaincode can invoke \textit{SFTP} to transfer files in local off-state.

\subsubsection{Transaction Workflow}

%In Hyperledger Fabric, as shown in Fig.\ref{fig::framework}, a common transaction workflow is as follows: 1. A client proposes a transaction proposal to some peer nodes, i.e. endorsers, specified by the endorsement policy; 2. Endorsers execute the chaincode, sign the execution results, and return the results with corresponding signatures to the client as proposal responses; 3. If the returned execution results from different endorsers are the same, the client assembles a transaction and sends it to the orderer node. 4. The orderer node collects multiple transactions in the same time, bundles transactions into a new block, and distribute the new block to all peers including both endorsers and non-endorsers. 5. All peers validate the transactions in the received new block. If the transaction is valid, the peer will update world state according to execution results. After validating all transactions, each peer appends the new block to a blockchain. 

In our three-phase file sharing event, one event involves four transactions as shown in Fig. \ref{fig::Module2}. All involved transactions follow the same common transaction workflow. The only difference is that endorsers are different in Steps 1 and 2. according to different endorsement policy setting. 


\subsection{Endorsement Policy Setting}
\label{sec::Endorsement_Policy_Set}

We illustrate the endorsement policy setting for involved four transactions in one file sharing event, including ``Tx: request permission", ``Tx: transfer file", ``Tx: request key" and ``Tx: decrypt file". The default chaincode-level endorsement policy is set as AND(Org1MSP, Org2MSP), which means peer nodes from both org1 and org2 need endorse a transaction. Note that org3 does not involve in any endorsing and only synchronizes the ledger data, i.e. world state and blockchain. In the following illustration, we assume Peer1 is the sender and Peer2 is the receiver.

% \subsubsection{File Uploading Event}
% In Module 1, when add a new file to the off-state, the smart contract should record the File Profile entry to the world state. The corresponding entry is $\langle$file\_name, $H(F)$, owner, access\_rule, description$\rangle$. The smart contract should read the file from the off-state and calculate the file hash. Since peer nodes only maintains their own files, only the file's owner peer can get the hash information. So the key-level policy for this entry should be customized. For example, when the user add file 1 to the Peer 1, the key-level policy for file 1 profile entry should be AND(Org1MSP), which mean only Peer 1 acts as the endorser and execute the smart contract. Though other peer nodes do not execute the smart contract, they will also store the entry in the world state and store the corresponding transaction in the blockchain. 

% \subsubsection{Module 2 implementation}
% Transferring files involves three phases:

\subsubsection{Tx: request permission}
During this transaction, chaincode verifies if pre-defined access control rules are satisfied, and records the verification result in an \texttt{Event} entry. This should be conducted by both sender and receiver, i.e. Peer1 and Peer2. So the endorsement policy for this transaction uses the default chaincode-level endorsement policy, i.e. AND(Org1MSP, Org2MSP). 

\subsubsection{Tx: file transfer}
During this transaction, chaincode conducts encrypting file, transferring file and writing \texttt{Encryption Key} to world state. $K_{aes}$ in \texttt{Encryption Key} should be kept only by the sender and other peers only store the hash. So \texttt{Encryption Key} should be set as a PDC and only the sender node Peer1 is the PDC member. Besides, only Peer1 owns the file to be encrypted and transfered. So the endorsement policy for this transaction should be customized as a collection-level policy and the policy should be AND(Org1MSP). That's only Peer1 performs as an endorser.

\subsubsection{Tx: request key}
During this transaction, chaincode should reset the PDC member of \texttt{Encryption Key} and add the receiver Peer2 to the PDC member. Then the receiver will own the original $K_{aes}$. The sender Peer1 should act as the endorser since it is the only original member of \texttt{Encryption Key}. The endorsement policy for this transaction should be AND(Org1MSP).

\subsubsection{Tx: query key and decrypt}
During this transaction, chaincode queries \texttt{Encryption Key} in world state to decrypt the encrypted file in the off-state. It is the receiver Peer2 who needs to decrypt the received encrypted file. And Peer2 now owns $K_{aes}$. So the endorsement policy for this transaction should be set as AND(Org2MSP).

% \subsubsection{Stage 3 implementation}

% If some disputes occur, the auditer organization will involved. The audit organizaton does not involve in the file uploading and file transferring. It only records all entries in its world state and all transactions in its blockchain. The auditer peer only conducts audit. So the smart contract running in the Peer 3 is different from Peer 1 and Peer 2. This can be implemented due to the customizable smart contracts feature in Hyperledger Fabric. According to the three audit policies in Section \ref{sec::stage3}, the smart contract needs query the file profile entry, encryption key entry and the transaction history. All these information locates in the auditer peer node, so the endorsement policy can be set as AND(Org3MSP).

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{figures/fig_framwork.pdf}
\caption{Framework of big files sharing system based on Hyperledger Fabric
\Fu{Font too small. Shall be similar to body text font size}}
\label{fig::framework} 
\end{figure}

% \subsection{Big Files Sharing Workflow}

%The whole file transfer process involves multiple transactions. At stage 1, the client proposes a transaction to record the new file uploaded to the off-state. 
%At stage 2, the receiver's client first proposes a transaction to request the transfer agreement. Then the sender's client proposes a transaction to transfer the file from one node to the other node. Next the receiver's client proposes a transaction to request the encryption key and at last proposes another transaction to query the encryption key and decrypt the received file. 
%At stage 3, the client can propose a transaction to conduct one policy check according to different scenarios.



%All involved transactions in the whole file transfer process follow the same common transaction workflow in Hyperledger Fabric. The only difference is that the corresponding endorsement policy involved in different transactions are different since these transactions operate different entries in the world state. We have analysed the endorsement policy setting for different entries in the last Section \ref{sec::systemFramework}. The common transaction workflow is as following: i) The client proposes a transaction proposal to the endorsers defined by the endorsement policy; ii) Endorsers execute the smart contract, sign the execution results, and return the results with corresponding signatures to the client; iii) If the returned results from different endorsers are the same, the client assembles a transaction and sends it to the orderer node. iv) The orderer node collects multiple transactions in the same time, blindly bundles transactions into new blocks, and distribute the new block to all peers including both endorsers and non-endorsers. v) All peers validate the transactions in the received new block. If the transaction is valid, the peer will update the data in the world state and append the new block to the blockchain. 
